Exploiting Frequency Correlation for Hyperspectral Image Reconstruction

Deep priors have emerged as potent methods in hyperspectral image (HSI) reconstruction. While most methods emphasize space-domain learning using image space priors like non-local similarity, frequency-domain learning using image frequency priors remains neglected, limiting the reconstruction capability of networks. In this paper, we first propose a Hyperspectral Frequency Correlation (HFC) prior rooted in in-depth statistical frequency analyses of existent HSI datasets. Leveraging the HFC prior, we subsequently establish the frequency domain learning composed of a Spectral-wise self-Attention of Frequency (SAF) and a Spectral-spatial Interaction of Frequency (SIF) targeting low-frequency and high-frequency components, respectively. The outputs of SAF and SIF are adaptively merged by a learnable gating filter, thus achieving a thorough exploitation of image frequency priors. Integrating the frequency domain learning and the existing space domain learning, we finally develop the Correlation-driven Mixing Domains Transformer (CMDT) for HSI reconstruction. Extensive experiments highlight that our method surpasses various state-of-the-art (SOTA) methods in reconstruction quality and computational efficiency.

==> table/HFC.tex <==
\begin{wraptable}{r}{0.45\textwidth}
    \vspace{-10mm}
    \centering
    \caption{\small HFC metrics.}
    \vspace{2mm}
    \scalebox{0.7}{
        \begin{tabular}{c c c c}
        		%\small
        		\toprule
                    \rowcolor{lightgray}
        		metric &~~~~HFC~~~~ \\
        		\midrule
                Inference Time (s) &0.0592\\
                Computation Effort (GFlops) &0.498\\
                Memory Cost (M) &0.086\\
        		\bottomrule
        \end{tabular}
    }
    \label{tab:HFC}
    \vspace{-5mm}
\end{wraptable}

==> table/Kernelsize2.tex <==
% \begin{table}[!htbp]
%     \centering
%     \scalebox{0.8}{
%         \begin{tabular}{c c c  c c c c}
%         		%\small
%         		\toprule
%         		 model  & Baseline-3 & kernel-2 \\
%         		\midrule
%                 baseline-3  & 34.00 & 0.933 \\
%         		2  & 34.25 & 0.934 \\
%         		4 & 34.57 & 0.939 \\
%         		8 & \bf34.61 & \bf0.940 \\
%                     16 & 34.38 & 0.936 \\
%         		\bottomrule
%         \end{tabular}
%     }
%     \vspace{-0.2cm}
%     \caption{\small Ablation of various kernel sizes.}
%     \label{tab:kernelsize}
%     \vspace{-0.3cm}
% \end{table}

\begin{table}[tp]
    \caption{\small Ablation Study of Kernel Size in SAF.}
    \centering
    \scalebox{0.8}{
        \begin{tabular}{c c c  c c c c}
        		%\small
        		\toprule
                    % \rowcolor{lightgray}
        		  model & Baseline-3 & kernel-2 & kernel-4 & kernel-8 & kernel-16\\
        		\midrule
                    PSNR & 34.00 & 34.25 & 34.57 & \bf{34.61} & 34.38\\
        		SSIM & 0.930 & 0.934 & 0.939 & \bf{0.940} & 0.936\\
        		\bottomrule
        \end{tabular}
    }
    % \vspace{-0.2cm}
    \label{tab:kernelsize}
    \vspace{-0.3cm}
\end{table}

==> table/RDLUF.tex <==
\begin{wraptable}{r}{0.47\textwidth}
    \vspace{-12mm}
    \centering
    \caption{\small Fair comparison with RDLUF.}
    \vspace{2mm}
    \scalebox{0.68}{
        \begin{tabular}{c c c  c c c c}
        		%\small
        		\toprule
                    \rowcolor{lightgray}
        		~~stage~~ & ~~Ours~~ & ~~RDLUF~~ & ~~Ours-plus~~\\
        		\midrule
        		\multirow{2}{*}{$3$} & 36.01 & 21.81 & 35.15\\
                    \multirow{2}{*}{} & 34.68 & 0.558 & 0.390 \\
                \midrule
        		\multirow{2}{*}{$5$} & 36,78 & 15.13 & 27.06 \\
                    \multirow{2}{*}{} & 35.35 & 0.208 & 0.726 \\
                    \midrule
                    \multirow{2}{*}{$9$} & 36.45 & 12.20 & 24.22 \\
                    \multirow{2}{*}{} & 45.35 & 0.093 & 0.632 \\
        		\bottomrule
        \end{tabular}
    }
    \label{tab:rdlufcomp}
    \vspace{-6mm}
\end{wraptable}

==> table/SAM2.tex <==
\begin{table}[tp]
    \caption{\small Ablation Study of self-attention mechanisms.}
    \centering
    \scalebox{0.73}{
        \begin{tabular}{c c c  c c c c}
        		%\small
        		\toprule
                    \rowcolor{lightgray}
        	  model & Complexity & Params $(M)$ & FLOPs $(G)$ & PSNR & SSIM\\
        		\midrule
        		Baseline-2 & - & 0.4 & 6.85 & 32.79 & 0.904\\
        		G-MSA & $O(H^2W^2C)$ & 0.48& 10.3 & 33.63 & 0.920\\
        		SW-MSA  & $O(2K^2HWC)$ & 0.48 & 9.41 & 33.75 & 0.924\\
                    % S-MSA  & $O(HWC^2)$ & 0.48 & 8.89 & 33.82 & 0.926\\
                    HS-MSA  & $O(K^2HWC)$ & 0.48 & 9.72 & 34.05 & 0.930\\
                % SDLB & 6.85 & 0.48 & 9.72 & 8.89 & 9.72\\
                SAF & $O(HWC^2)$ & \bf0.48 & \bf7.87 & \bf34.61 & \bf0.940\\
        		\bottomrule
        \end{tabular}
    }
    % \vspace{-0.2cm}
    \label{tab:table5}
    \vspace{-0.3cm}
\end{table}

==> table/allbranches2.tex <==
\begin{table}[tp]
    \centering
    \caption{\small Break-down ablation of frequency domain learning.}
    \scalebox{0.78}{
        \begin{tabular}{c c c c c c c c}
        		%\small
        		\toprule
                    \rowcolor{lightgray}
        		Baseline-1  & SAF & SIF & Params$(M)$ & FLOPs$(G)$ & PSNR & SSIM\\
        		\midrule
        		\checkmark  &  &  & 0.55 & 16.30 & 36.02 & 0.952\\
                \checkmark  & \checkmark &  & 0.64 & 20.06 & 37.10 & 0.960\\
        		\checkmark  & \checkmark & \checkmark & 0.90 & 21.39 & \bf37.44 & \bf0.963\\
        		\bottomrule
        \end{tabular}
    }
    % \vspace{-0.2cm}
    \label{tab:table3}
    \vspace{-0.3cm}
\end{table}

==> table/selfattention.tex <==
\begin{wraptable}{r}{0.5\textwidth}
    % \vspace{-6mm}
    \centering
    \caption{\small Ablation of various self-attention mechanisms.}
    \vspace{2mm}
    \scalebox{0.73}{
        \begin{tabular}{c c c  c c c c}
        		%\small
        		\toprule
                    \rowcolor{lightgray}
        	  model & Complexity & Params $(M)$ & FLOPs $(G)$ & PSNR & SSIM\\
        		\midrule
        		Baseline-2 & - & 0.4 & 6.85 & 32.79 & 0.904\\
        		G-MSA & $O(H^2W^2C)$ & 0.48& 10.3 & 33.63 & 0.920\\
        		SW-MSA  & $O(2K^2HWC)$ & 0.48 & 9.41 & 33.75 & 0.924\\
                    % S-MSA  & $O(HWC^2)$ & 0.48 & 8.89 & 33.82 & 0.926\\
                    HS-MSA  & $O(K^2HWC)$ & 0.48 & 9.72 & 34.05 & 0.930\\
                % SDLB & 6.85 & 0.48 & 9.72 & 8.89 & 9.72\\
                SAF & $O(HWC^2)$ & \bf0.48 & \bf7.87 & \bf34.61 & \bf0.940\\
        		\bottomrule
        \end{tabular}
    }
    \label{tab:selfattention}
    \vspace{-3mm}
\end{wraptable}

==> table/sharing.tex <==
\begin{wraptable}{r}{0.5\textwidth}
    % \vspace{-6mm}
    \centering
    \caption{\small Ablation study of parameter sharing.}
    \vspace{2mm}
    \scalebox{0.65}{
        \begin{tabular}{c c c c c}
				\toprule
				\rowcolor{color3}stages &~Params (M)~ &~FLOPs (G)~ &~PSNR~ & ~SSIM~   \\
				%\rowcolor{color3} &\cite{edvr} &\cite{Su} &\cite{stfan}  &\cite{tsp}  &\textbf{(Ours)} \\
				\midrule
				2 &1.75   &21.39 &\bf37.64  &\bf 0.966  \\
				2-shared  &0.90    &21.39  &37.44 &0.963  \\
				3  &2.60    &31.56  &38.05  &0.967 \\
				3-shared &0.90    &31.56  &\bf38.16 &\bf0.968  \\
                5  &4.31    &51.90  &38.42  &0.971 \\
				5-shared  &0.90    &38.42  &\bf38.96 &\bf0.974  \\
				\bottomrule
	\end{tabular}}
    }
    \label{tab:sharing}
    \vspace{-3mm}
\end{wraptable}
